Evaluating the Effectiveness of Margin Parameter when Learning Knowledge Embedding Representation for Domain-specific Multi-relational Categorized Data

Learning knowledge representation is an increasingly important technology that supports a variety of machine learning related applications. However, the choice of hyperparameters is seldom justified and usually relies on exhaustive search. Understanding the effect of hyperparameter combinations on embedding quality is crucial to avoid the inefficient process and enhance practicality of vector representation methods. We evaluate the effects of distinct values for the margin parameter focused on translational embedding representation models for multi-relational categorized data. We assess the margin influence regarding the quality of embedding models by contrasting traditional link prediction task accuracy against a classification task. The findings provide evidence that lower values of margin are not rigorous enough to help with the learning process, whereas larger values produce much noise pushing the entities beyond to the surface of the hyperspace, thus requiring constant regularization. Finally, the correlation between link prediction and classification accuracy shows traditional validation protocol for embedding models is a weak metric to represent the quality of embedding representation.

==> KER-LM-5-Discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Discussion}
%\label{SECTION:Discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%- You can try to calculate correlation between MLP accuracy and max cycle (I didn't yet) , but if the result is < 0 (negative) that means when the model finds the best solution earlier when the LM is adequately set, otherwise higher LM will be pushing the training process longer but with enough noise to avoid improving the quality of the result embedding representation.
%Cycle has strong correlation with MLP accuracy on some dimensions of certain datasets, but there is no obvious trend 

%For \textit{Mushroom} which is simpler than other datasets that it only contains N-to-1 relations, the cycle... no correlation...

%For more complex KGs eg. \textit{Freebase}, there appears to be a stronger negative correlation between the convergence cycle and classification accuracy...


% In each dataset, the set of entity types considered for each ontology-based constraint differs.
%

